Does CLIP's Generalization Performance Mainly Stem from High Train-Test Similarity?

Foundation models like CLIP are trained on hundreds of millions of samples and effortlessly generalize to new tasks and inputs. Out of the box, CLIP shows stellar zero-shot and few-shot capabilities on a wide range of out-of-distribution (OOD) benchmarks, which prior works attribute mainly to today's large and comprehensive training dataset (like LAION). However, it is questionable how meaningful terms like out-of-distribution generalization are for CLIP as it seems likely that web-scale datasets like LAION simply contain many samples that are similar to common OOD benchmarks originally designed for ImageNet. To test this hypothesis, we retrain CLIP on pruned LAION splits that replicate ImageNet's train-test similarity with respect to common OOD benchmarks. While we observe a performance drop on some benchmarks, surprisingly, CLIP's overall performance remains high. This shows that high train-test similarity is insufficient to explain CLIP's OOD performance, and other properties of the training data must drive CLIP to learn more generalizable representations. Additionally, by pruning data points that are dissimilar to the OOD benchmarks, we uncover a 100M split of LAION ($\frac{1}{4}$th of its original size) on which CLIP can be trained to match its original OOD performance.

==> 04_difficulty.tex <==
\section{The similarity hypothesis}\label{sec:difficulty}
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/Fig2.pdf}
    \caption{
        \textbf{Relation between \textit{perceptual similarity} and visual closeness of nearest neighbors}. Query images are sampled from \imagenets{} (top row) and are connected to their nearest neighbor in \laionfour{} (bottom row). As in Fig.~\ref{fig:motivation}, perceptual similarity is simply the cosine similarity measured in CLIP's image embedding space.}
    \label{fig:fig2}
\end{figure}



\subsection{Comparing LAION and ImageNet’s test-set similarity}\label{sec:analysis}
The popular \imagenetk{} and \laionfour{} datasets differ not only in scale but also in diversity.
\imagenetk{} consists of \SI{1.2}{million} samples, the vast majority of which are natural images. In comparison, \laionfour{} comprises roughly \SI{400}{million} samples scraped from the Common Crawl dataset\footnote{\url{ https://commoncrawl.org/}}. Common Crawl comprises petabytes of data collected over more than a decade of web crawling; \laionfour{}, therefore, contains an extremely high diversity and density of images.

The most common datasets used for testing OOD generalization performance are \imagenets{}, \imagenetr{}, \imagenetvtwo{}, \imageneta{}, and \objectnet{}.
To quantify similarity of samples from the aforementioned datasets to data points in \imagenetk{} (for which they were designed) and  \laionfour{}, we here use a common \textit{perceptual similarity} metric based on the cosine similarity in the image embedding space of a \laionfour{}-trained \vitbsixteenp{} model~\citep{ilharco_gabriel_2021_5143773}.
\citet{abbas2023semdedup} demonstrated that nearest neighbors in the image embedding space share \textit{semantic} and \textit{stylistic} characteristics. We illustrate this in Fig.~\ref{fig:fig2}, where we plot samples from \imagenets{} and their neighbors in \laionfour{} for different similarity values. Visually, the similarity scores correlate well with the semantic and stylistic closeness of the image pairs. This is corroborated by other works that demonstrate high perceptual alignment between CLIP's embedding similarity and human perception \citep{dreamsim} and use it to sample \imagenet{}-like data points from a large dataset \citep{datacomp} or to build a similarity-based classifier for few-shot classification \citep{tipadapter}. We consequently use it as the main similarity measure throughout this paper. We interchangeably use the terms \textit{similarity} and \textit{perceptual similarity} to refer to this metric. Likewise, \emph{nearest neighbors} or \emph{similar images to a query image} denotes the closest images (images with the highest similarity) in the CLIP image-embedding space.
\begin{figure}[tb]
    \centering
    \includegraphics[width=\textwidth]{figures/Fig3_histograms.pdf}
    \caption{
        \textbf{Similarity of nearest neighbors to test sets varies between \laionfour{} and \imagenett{} and is correlated with performance}.
        \textbf{Left}: The histograms display the similarity of samples in \imagenets{} (left), \imagenetr{} (center), and \imagenetv{} (right) to their nearest neighbors in \laionfour{} (red) and \imagenett{} (blue). \laionfour{} is overall more similar to \imagenets{} and \imagenetr{}, while \imagenett{} is more similar to \imagenetv{}.
        \textbf{Right}: The strong correlation between perceptual similarity of test points to nearest neighbors in \laionfour{} samples and CLIP's top-1 classification accuracy indicates that differences in similarity can be expected to drastically impact the performance of LAION-trained models. Data points in the correlation plot are averaged over bins (interval = 0.05) of the red histograms in the left plot.
    }\label{fig:fig3}
\end{figure}

In Fig.~\ref{fig:motivation} and Appx.~\ref{sec:appendix-nn_vis}, we use perceptual similarity to illustrate that often nearest neighbors of samples from OOD datasets in \laionfour{} are semantically and stylistically more similar to them than their nearest neighbors from \imagenett{} are. Specifically, for \imagenets{} and \imagenetr{} images, it is evident that neighbors in \laionfour{} share both semantics and style, whereas neighbors in \imagenett{} are merely natural images of the same class. In contrast, for \imagenetv{}, nearest neighbors in \imagenett{} seem more similar than the neighbors in \laionfour{}. 
To quantify this observation, we measure the distribution of perceptual similarities of all \imagenets{} samples to their nearest neighbors in \laionfour{} and \imagenett{} (Fig.~\ref{fig:fig3}, left). While \imagenett{}'s similarity distribution has a mode of roughly 0.65 and is fairly narrow, LAION's similarity distribution peaks at around 0.8 and is much broader. The same trend can be observed for \imagenetr{}. In contrast, the distribution of nearest-neighbor similarities to \imagenetv{} (Fig.~\ref{fig:fig3}, right) indicates that samples are generally closer to \imagenett{} than to the \laionfour{}, but the difference in modes is smaller. We refer the reader to Appx.~\ref{sec:appendix-nn_vis}~and~\ref{sec:appendix-nn_sims} for nearest neighbor and perceptual similarity histograms for \imagenetvtwo{}, \imageneta{}, and \objectnet{}.
For these datasets, the similarity distributions of \laionfour{} and \imagenett{} barely differ.

Moreover, in Appx.~\ref{sec:appendix-duplicates}, we detail the number of \emph{near duplicates} (duplicates up to small shifts or crops) of the OOD datasets in \laionfour{} and \imagenett{}. While we found \SI{3.1}{\%} of \imagenets{} images to have duplicates in \laionfour{}, there are only \SI{0.04}{\%} \imagenets{} duplicates in \imagenett{}. On the other hand, \imagenett{} contains duplicates of \SI{2.67}{\%} \imagenetv{} images as opposed to just \SI{0.14}{\%} \imagenetv{} images  in \laionfour{}.

The rightmost plot of Fig.~\ref{fig:fig3} illustrates that similarity between test samples and their nearest neighbors is a good predictor for a model's performance on these samples. Each data point here corresponds to a bin from one of the red histograms to the left. We report CLIP's average top-1 classification accuracy over all samples in the same bin. We observe a clear correlation between similarity and classification performance, ranging from \SI{35}{\%} accuracy for sketches that have no similar counterparts in \laionfour{} (similarity 0.38) up to \SI{69}{\%} accuracy for sketches that are duplicated in \laionfour{} (similarity close to 1). 

Based on these observations, we expect that for \imagenets{} and \imagenetr{}, \laionfour{} will contain a large number of highly similar images. Because of the high correlation between train-test similarity and accuracy, it is a natural hypothesis that this similarity largely explains CLIP's high performance.



% \subsection{Impact of pruning (dis)similar images}\label{sec:near_far}
% In the last subsection, we found that a sample's similarity to its nearest neighbors in the training set is highly predictive of a model's performance on this sample. We can observe this effect more directly by pruning \textit{similar} samples from LAION in order of decreasing perceptual similarity to test data points. We then train CLIP on the pruned dataset and evaluate its performance on the test set to see how much CLIP's performance is influenced by train-test set similarity. To elucidate further, we order all samples in LAION by their similarity to the perceptually most similar test sample from a given test set. We then start pruning from those samples in LAION that are most similar to the test set in the decreasing order of similarity. To ease analysis, we perform this experiment on \laiontwo{} (see Sec.~\ref{sec:exp_details}). We prune the dataset to 150M, 100M, and 50M (collectively called `near-pruned' splits), making the splits progressively more dissimilar to the test sets.
% %
% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=\textwidth]{figures/Fig5_ICLR_reverse.pdf}
%     \caption{\textbf{Effect of pruning similar and dissimilar points to a given test set}. The baseline model is trained on de-duplicated \laionfour{}, which we call \laiontwo{}. To generate the `near-pruned' datasets, we remove images in decreasing order of similarity to \imagenets{} or \imagenetv{} (based on CLIP image-embedding similarity). In contrast, the `far-pruned' datasets are generated by pruning images in the increasing order of similarity values to the respective test sets. For the `rand-pruned' datasets, we prune random points. Pruning similar images adversely affects performance compared to pruning dissimilar or random images. CLIP's `near-pruned' and `far-pruned' performance across all six test sets is shown in Fig.~\ref{fig:near_far_appendix}.}
%     \label{fig:pruning_v_performance}
% \end{figure}

% We also examine the effect of removing points from \laiontwo{} that are highly \emph{dissimilar} to the test data points.
% We refer to the resulting datasets as `far-pruned'. Here again, we order all samples in LAION by
% their similarity to the perceptually most similar test sample from a given test set. We then start pruning from those samples in LAION that are least similar to the test set in increasing order of similarity. As a baseline, we also prune random points to generate `rand-pruned' data splits. We separately use \imagenets{} and \imagenetv{} as test datasets to generate `near-pruned' and `far-pruned' splits.

% We train CLIP on 15 different subsets of \laiontwo{} which differ in their pruning strategy (`near-pruned', `far-pruned', or `rand-pruned'), the target test set (\imagenetv{} or \imagenets{}) and their pruning strength (150M, 100M, and 50M). We plot the resulting zero-shot accuracy on the target test sets in Fig.~\ref{fig:pruning_v_performance}. We find that the `near-pruned' accuracy curve drops quickly with decreasing dataset size. This reiterates that a large chunk of CLIP's performance directly stems from similar images to the test set that are removed here. In contrast, the performance of models trained on the `far-pruned' datasets remains stable up until a dataset size of 100M. In fact, the performance even slightly surpasses that of the baseline model, further indicating that dissimilar samples do not contribute to CLIP's performance and instead act more like noise in the training data. We extend our analysis in Appx.~\ref{sec:appendix:near_far} (Fig.~\ref{fig:near_far_appendix}). We also extend our analysis to \imagenett{} in Appx~\ref{sec:appendix-near_far_imagenet}.

% Motivated by the performance increase of CLIP trained on `far-pruned' datasets, we aim to build a `coreset' of smaller size that consists ofsamples needed to generalize well to the six test sets. To this end, we far-prune \laiontwo{} based on all six test sets to obtain an `all-pruned' dataset of size 100M. In other words, we remove samples from \laiontwo{} that are highly dissimilar to all samples in the six OOD datasets we consider. A CLIP model trained on the `all-pruned' dataset performs significantly better than a CLIP model trained on a de-duplicated dataset of size 100M \cite{ilharco_gabriel_2021_5143773} and roughly matches the performance of a \laiontwo{} trained model (see Fig.~\ref{fig:pruning_v_performance} \& Appx.~\ref{sec:appendix:coreset}).



\subsection{Impact of pruning (dis)similar images}\label{sec:near_far}
In the last subsection, we found that a sample's similarity to its nearest neighbors in the training set is highly predictive of a model's performance on this sample. We can observe this effect more directly by pruning \textit{similar} samples from LAION in order of decreasing perceptual similarity to test data points. We then train CLIP on the pruned dataset and evaluate its performance on the test set to see how much CLIP's performance is influenced by train-test set similarity. To elucidate further, we order all samples in LAION by their similarity to the perceptually most similar test sample from a given test set. We then start pruning from those samples in LAION that are most similar to the test set in the decreasing order of similarity. To ease analysis, we perform this experiment on \laiontwo{} (see Sec.~\ref{sec:exp_details}). We prune the dataset to 150M, 100M, and 50M (collectively called `near-pruned' splits), making the splits progressively more dissimilar to the test sets.
%
\begin{figure}[tb]
    \centering
    \includegraphics[width=\textwidth]{figures/Fig5_ICLR_reverse.pdf}
    \caption{\textbf{Effect of pruning similar and dissimilar points to a given test set}. The baseline model is trained on de-duplicated \laionfour{}, which we call \laiontwo{}. To generate the `near-pruned' datasets, we remove images in decreasing order of similarity to \imagenets{} or \imagenetv{} (based on CLIP image-embedding similarity). In contrast, the `far-pruned' datasets are generated by pruning images in the increasing order of similarity values to the respective test sets. For the `rand-pruned' datasets, we prune random points. Pruning similar images adversely affects performance compared to pruning dissimilar or random images. CLIP's `near-pruned' and `far-pruned' performance across all six test sets is shown in Fig.~\ref{fig:near_far_appendix}.}
    \label{fig:pruning_v_performance}
\end{figure}

We also examine the effect of removing points from \laiontwo{} that are highly \emph{dissimilar} to the test data points.
We refer to the resulting datasets as `far-pruned'. Here again, we order all samples in LAION by
their similarity to the perceptually most similar test sample from a given test set. We then start pruning from those samples in LAION that are least similar to the test set in increasing order of similarity. As a baseline, we also prune random points to generate `rand-pruned' data splits. We separately use \imagenets{} and \imagenetv{} as test datasets to generate `near-pruned' and `far-pruned' splits.

We train CLIP on 15 different subsets of \laiontwo{} which differ in their pruning strategy (`near-pruned', `far-pruned', or `rand-pruned'), the target test set (\imagenetv{} or \imagenets{}) and their pruning strength (150M, 100M, and 50M). We plot the resulting zero-shot accuracy on the target test sets in Fig.~\ref{fig:pruning_v_performance}. We find that the `near-pruned' accuracy curve drops quickly with decreasing dataset size. This reiterates that a large chunk of CLIP's performance directly stems from similar images to the test set that are removed here. In contrast, the performance of models trained on the `far-pruned' datasets remains stable up until a dataset size of 100M. In fact, the performance even slightly surpasses that of the baseline model, further indicating that dissimilar samples do not contribute to CLIP's performance and instead act more like noise in the training data. We extend our analysis in Appx.~\ref{sec:appendix:near_far} (Fig.~\ref{fig:near_far_appendix}). We also extend our analysis to \imagenett{} in Appx~\ref{app:near_far_imagenet}.

Motivated by the performance increase of CLIP trained on `far-pruned' datasets, we aim to build a `coreset' of smaller size that consists of samples needed to generalize well to the six test sets. To this end, we far-prune \laiontwo{} based on all six test sets to obtain an `all-pruned' dataset of size 100M. In other words, we remove samples from \laiontwo{} that are highly dissimilar to all samples in the six OOD datasets we consider. A CLIP model trained on the `all-pruned' dataset performs significantly better than a CLIP model trained on a de-duplicated dataset of size 100M \cite{ilharco_gabriel_2021_5143773} and roughly matches the performance of a \laiontwo{} trained model (see Fig.~\ref{fig:pruning_v_performance} \& Appx.~\ref{sec:appendix:coreset}).

==> 05_gg.tex <==
\section{similarity gap}\label{sec:benchmarking}

% intro to more formal approach
In Sec.~\ref{sec:difficulty}, we provide direct and indirect evidence that CLIP's performance on common OOD test sets might mainly stem from images in its training set that are \emph{highly similar} to the test sets. We now aim to control for this confounder more systematically. To this end, we note that even for \imagenett{}, the perceptual similarity between OOD test samples and their most similar training sample differs across test samples. Our goal is to prune LAION so that the pruned dataset replicates the perceptual similarities between test samples and \imagenett{}.
We formalize this notion as \emph{similarity gap} below.
% and explain how to use it as a systematic measure to study generalization performance more fairly, even in the age of massive web-scale training datasets.

%We vaguely defined \emph{highly similar images} in Sec.~\ref{sec:intro} as images that are more similar to a given test set than any sample \imagenetk{}. We now formalize \emph{similarity gap} as a measure of train-test similarity between datasets that is independent of dataset scale and diversity and can be used to systematically define highly similar images.

% We now formalize how to capture the discrepancy in test-set similarity of various training sets, so as to train and evaluate CLIP in a fairer way. We propose a systematic approach to correct this discrepancy, which ensures that the test set is equivalently far removed from both the train sets.

% introduce basic notation and similarity function
Let us consider two training datasets, denoted as $\mathcal{D}_S$ (small, like \imagenett{}) and $\mathcal{D}_L$ (large, like \laionfour{}), along with a test dataset $\mathcal{T}$ (like ImageNet-Sketch). For the sake of simplicity, we assume that $\mathcal{D}_S$ is a subset of $\mathcal{D}_L$. We choose a similarity measure $s(\cdot,\cdot): \mathcal{T}\times\mathcal{D}\to \mathbb{R}^{+}$ in order to find the $k$ nearest neighbors in the training set for each sample $t_i\in\mathcal{T}$. Although we choose $k=1$ for simplicity, the approach can be generalized straightforwardly. We denote the nearest-neighbor similarity between $t_i$ and a dataset $\mathcal{D}$ as $s_i(\mathcal D)$, which is given by
%
\begin{equation}
s_i(\mathcal{D}) = \max_{x\in\mathcal{D}} s(t_i, x).
\end{equation}
%
The set of nearest-neighbor similarities
%
\begin{equation}
    S(\mathcal D, \mathcal T) = \left\{s_i(\mathcal{D}) \mid i \in \big[1, \left|\mathcal{T}\right| \big] \right\}
\end{equation}
%
then quantifies the \textit{similarity gap} $S$ between training and test set. We can think of this measure as a full characterization of the training set's similarity to any point in the test set; compare Fig.~\ref{fig:method}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig4_v3.pdf}
    \caption{
        \textbf{Aligning the similarity gap of two datasets}.
        A larger, denser, more diverse dataset likely contains samples more similar to given test points than a smaller, sparser one. To control for this, we compute the nearest-neighbor similarity of each test point to the smaller dataset (left) and prune points from the larger dataset that lie within this hull (center). We end up with a corrected large dataset replicating the \textit{similarity gap} of the small one (right).
    }\label{fig:method}
\end{figure}

% explain how large dataset is pruned
Based on the assumption that the large dataset contains all samples from the small dataset, it follows that $s_i(\mathcal{D}_S) \leq s_i(\mathcal{D}_L)$. In other words, the nearest-neighbor similarity to samples in the small training set is always smaller than or equal to the similarity to samples in the large training set. Consequently, on a per-sample basis, $S(\mathcal D_L, \mathcal T)$ is strictly larger than $S(\mathcal D_S, \mathcal T)$, \ie, the large dataset is generally more similar to the test than the small dataset. We aim to identify a maximally large subset $\tilde{\mathcal{D}}_L\subseteq\mathcal{D}_L$ of the large training set, such that its similarity gap $S(\mathcal{\tilde D}_L, \mathcal T) = S(\mathcal D_S, \mathcal T)$ is equal to the small dataset (on a per-sample basis, meaning $s_i(\mathcal{\tilde D}_S) = s_i(\mathcal{D}_S)$ for all samples).
To achieve this, we examine each test sample $t_i$ and remove any sample $x\in \mathcal{D}_L$ for which the similarity $s(t_i, x) > s_i(\mathcal{D}_S)$.
We illustrate this procedure in Fig.~\ref{fig:method}. Sec.~\ref{sec:experiments} applies this framework to \laionfour{} and \imagenett{}. We compute perceptual similarities in the embedding space of pretrained \vitbsixteenp{}. This ensures that we remove all data points in LAION that are semantically and stylistically more similar to the test data points than samples in \imagenett{}. In this way, we obtain a version of \laionfour{} that is equally far removed from the test sets as \imagenett{}.


